PoNQ: a Neural QEM-based Mesh Representation

Although polygon meshes have been a standard representation in geometry processing, their irregular and combinatorial nature hinders their suitability for learning-based applications. In this work, we introduce a novel learnable mesh representation through a set of local 3D sample Points and their associated Normals and Quadric error metrics (QEM) w.r.t. the underlying shape, which we denote PoNQ. A global mesh is directly derived from PoNQ by efficiently leveraging the knowledge of the local quadric errors. Besides marking the first use of QEM within a neural shape representation, our contribution guarantees both topological and geometrical properties by ensuring that a PoNQ mesh does not self-intersect and is always the boundary of a volume. Notably, our representation does not rely on a regular grid, is supervised directly by the target surface alone, and also handles open surfaces with boundaries and/or sharp features. We demonstrate the efficacy of PoNQ through a learning-based mesh prediction from SDF grids and show that our method surpasses recent state-of-the-art techniques in terms of both surface and edge-based metrics.

==> tables/sdf_reach.tex <==
\begin{tabular}{|l|c|c|c|c|c|r|}
  \hline
  \textbf{Method}            & Grid & CD ($\times 10^{-5}$) & F1 & NC & ECD & EF1 \\
  \hline
  \hline
  Reach For the Spheres~\cite{sellan_reach_2023}  & $32^3$  & 1.836  &  0.805  &  0.934 & 0.155 & 0.235 \\
  PoNQ  & $32^3$  & 1.193  &  0.828  &  0.955 & 0.182 & 0.309    \\
  \hline
  Reach For the Spheres~\cite{sellan_reach_2023}  & $64^3$  & 1.506  &  0.889  &  0.957 & 0.139 & 0.347 \\
  PoNQ  & $64^3$  & 0.708  &  0.927  &  0.978 & 0.149 & 0.480 \\
  \hline
  Reach For the Spheres~\cite{sellan_reach_2023}  & $128^3$  & 6.438  &  0.901  &  0.963 & 0.161 & 0.386 \\
  PoNQ  & $128^3$  &  0.650  &  0.936  &  0.987 & 0.188 & 0.529 \\
  \hline
 
\end{tabular}

==> text/garbage.tex <==
From method.tex:

\subsubsection{Optimization-based 3D Reconstruction}
\label{sec:method_optim}

\nm{READ SECTION 4.2 FIRST. Should we move some stuff from there here? I think it's easier to explain the method for watertight shapes here and for open surfaces in the "experiment" section since it's more of an experiment.}
We utilize a similar setting than VoroMesh~\cite{maruani_voromesh_2023}: \pa{not sure we should cite VoroMesh here as this suggests too much the authors. or cite 2-3 papers that utilize a similar setting?} \nm{The code is public so it's really easy for anyone to reuse the same setting}
the input $X \in \mathbb{R}^{S \times 3}$ is a dense point sample of a watertight shape. % PA: verify consistency with above pb statement
Each sample $x$ is associated to an oriented normal $n(x)$. The predicted points $\mathbf{P}$ are initially placed on a regular grid around the ground truth samples. We optimize their position \nm{using the Chamfer distance as a loss function}: \pa{to me this is too fast, as you must explain how you optimize, too}
\begin{equation}
    CD(\mathbf{P}, X)=\frac{1}{|\mathbf{P}|} \sum_{\textbf{p} \in \mathbf{P}} \min_{x \in X} \|\textbf{p}-x\|^2 +  \frac{1}{|X|} \sum_{x \in X} \min_{\textbf{p} \in \mathbf{P}} \|\textbf{p}-x\|^2 
\end{equation}
We then compute sample-to-points correspondences:
\begin{align}
X(\textbf{p}) &= \{ x \in X \  | \ \|x-\textbf{p}\| \leq \| x-\textbf{q}\|, \forall \textbf{q} \in \mathbf{P}\} 
\end{align}
and obtain mean normals $\textbf{n}_p = \frac{1}{|X(\textbf{p})|} \sum_{x \in X(\textbf{p})} n(x) $
and QEM $\textbf{Q}_p = \left(\!\!\begin{smallmatrix}
\textbf{A}_p & -\textbf{b}_p\\
-\textbf{b}_p^T & \textbf{c}_p
\end{smallmatrix}\!\right)$  as defined in Equation~\ref{eq:qem}. 

We then compute the optimal vertex locations $\textbf{V}^*$ as $\textbf{v}^*_p = \textbf{A}_p^{-1} \textbf{b}_p$, and construct a mesh as detailed in Section~\ref{sec:method_meshing}. 
% PA: stick to only one term throughout the paper: either "point locations and vertex locations" or positions.

 ---------------

==> text/old_conclusion_old.tex <==
\section{Conclusion, Limitations and Future Works}
\label{sec:conclusion}

We proposed a novel learnable 3D shape representation, coined PoNQ which combines the power of the quadric error metric (QEM) originally devised for mesh decimation, and insights from computational geometry. PoNQ relies on points, normals, and QEM matrices to represent local geometric information, which are later leveraged to construct a triangle mesh that is guaranteed to be the boundary of a volume and devoid of self-intersections. We demonstrated the representation power of PoNQ through optimization-based tasks, and in learning-based reconstruction experiments, showing significant improvement upon previous 3D representations. We thus believe that PoNQ is poised to find many applications in neural shape processing.


While our neural PoNQ representation excels on learning tasks, there is still room for improvements.
Compared to SAP or VoroMesh, our network has to learn additional quadric information, thus incurring a higher network size. However we argue that it is not much of an issue in practice since $80\%$ of the learned parameters are concentrated in the shared encoder which contains the largest layers. Moreover, the task of fitting points, QEM and normals is quite straightforward and does not require overly large networks (e.g., VoroMesh requires 8.4M parameters while PoNQ only requires 2.7M). One could also argue that PoNQ may create non-manifold vertices of edges in degenerate situations -- for instance, if a 1-ring of a vertex contains two \textit{non-adjacent} tetrahedra that were both labeled as \emph{inside}. As suggested in~\cite{maruani_voromesh_2023}, however, in such cases, one can simply duplicate these few non-manifold elements and connect them to their neighboring mesh elements to enforce manifoldness.

A nice extension to our work could be to integrate the PoNQ representation in a differentiable rendering pipeline.
We also believe that our meshing of open boundaries can be further refined. In particular, the simplistic filtering we used to generate open meshes can likely be refined. Finally, as mentioned above, a hierarchical version of our PoNQ can potentially be especially exciting as flexible \textit{multi-scale} shape representation. \nm{We can do multi scale so I would rephrase this}



==> text/old_method_old.tex <==
\section{Method}
\label{sec:method}

We now delve into our PoNQ representation by first, in Sec.~\ref{sec:motivation}, offering a more in-depth introduction to QEM and how we use it. We then describe our representation in Sec.~\ref{sec:methodNQ} along with its use in learning tasks, and finally introduce our PoNQ mesh extraction approach in Sec.~\ref{sec:method_meshing}. 
%m@: we can also remove the Section numbers if you want.

%\vspace*{-2mm}

\subsection{Motivation: Quadric Error Metrics}
\label{sec:motivation}

Given a point $p_i  \in  \mathbb{R}^3$ and a normal $n_i \in \mathbb{R}^3$, the signed distance from a given location $x$ to the plane passing through $p_i$ that is normal to $n_i$ is given simply as $d_{p_i, n_i}(x) = (x\!-\!p_i)^t n_i$. The squared distance can thus be rewritten as $d_{p_i, n_i}(x)^2 = x^t A_i x - 2 b_i^t x + c_i$, where $3 \times 3$ matrix $A_i$, vector $b_i$, and scalar $c_i$ are defined as:\vspace*{-1.5mm}
\begin{equation}
    A_i = n_i n_i^t, \quad b_i = A_i p_i, \quad c_i = p_i^t A_i p_i. \vspace*{-1.5mm}
\end{equation}
Summing the squared distances to a \emph{set of planes} defined by $n$ point-normal pairs thus yields: \vspace*{-1.5mm}
\begin{align}
 \operatorname{QEM}(x) &= \sum\nolimits_{i=1..n} d^2_{x_i, n_i}(x) \nonumber\\
    & = x^t \underbracket{\bigl(\sum_i A_i \bigr)}_{\coloneqq A}  x - 2 {\underbracket{\bigl(\sum_i b_i\bigr)}_{\coloneqq b}} ^t x + \underbracket{\bigl(\sum_i c_i\bigr)}_{\coloneqq c} \label{eq:sumsAbc}\\
    & =  [x, 1]^t 
        \underbracket{\begin{pmatrix}
        A  & -b\\
        -b^t & c
        \end{pmatrix}}_{\coloneqq Q} [x, 1]. \label{eq:qem} 
\end{align}
Thus, the QEM matrix $Q \!\in\! \mathbb{R}^{4 \times 4}$ from Eq.~\eqref{eq:qem}, obtained by  simply summing the matrices $A_i$ as $A$, vectors $b_i$ as $b$, and scalars $c_i$ as c, concisely encodes the summed distances to a set of different planes. Assuming the submatrix $A$ to be invertible, 
%\in \mathbb{R}^{3 \times 3}$ is positive semi-definite and in general invertible. In this case
% and if it is not invertible -> svd but requires a query point
the quadratic $\operatorname{QEM}$ function reaches its unique minimum at a location $v^*\!=\! A^{-1} b$, and $\operatorname{QEM}(v^*) \!=\! c - b^t v^*$. 
Given that the matrix $Q$ offers a compact encoding of (an arbitrary number of) local tangent planes and a simple expression for where to place a vertex $v^*$ to stay optimally close to these planes, we leverage them as part of a powerful 3D \emph{representation} suitable for machine learning pipelines.

\subsection{PoNQ representation}
\label{sec:methodNQ}
We can now define how our representation is assembled given an input surface, before describing its integration within a learning pipeline. After that, we describe how this proposed choice of representation lends itself very naturally to an efficient meshing algorithm which robustly handles sharp features and can even be adapted to handle open surfaces with boundaries. In order to remove possible ambiguities, we will use a bold font to refer to different quantities involved in the PoNQ representation, i.e., what will be optimized or learned.

\subsubsection{QEM-based representation thru optimization}
\label{sec:method_rep}

The PoNQ representation consists in a set of \textbf{Po}ints augmented with their local \textbf{N}ormals and \textbf{Q}uadrics --- hence its name. We thus refer to entire set of point-normal-quadric data as $\boldsymbol{\mathcal{P}} = \{ (\mathbf{p}_i, \mathbf{n}_i, \mathbf{Q}_i)_{i=1 ... m}\}$,
where $\mathbf{p}_i \!\in\! \mathbb{R}^3, \mathbf{n}_i \!\in\! \mathbb{R}^3$, and $\mathbf{Q}_i \!\in\! \mathbb{R}^{4 \!\times\! 4}$ --- each of them either optimized to fit a single shape or learned by neural networks.

At first sight, our approach is similar to most point-based representation: we want to represent a watertight and non-self-intersecting input shape (finely discretized by samples $s_k$ with their local normals $n(s_k)$) with $m$ 3D points $\{\mathbf{p}_i\}_{i=1..m}$. We can initialize and optimize this point set in various ways. In an optimization-based setting, we initialize the points on a regular grid around the input shape (many other initializations work equally well), and optimize their position with respect to the input samples $\{s_k\}_k\!\coloneqq\!\mathcal{S}$ to minimize the bi-directional Chamfer Distance: \vspace*{-1.5mm}
\begin{align}
    \operatorname{CD}(\boldsymbol{\mathcal{P}},\mathcal{S})=&\frac{1}{|\boldsymbol{\mathcal{P}}|} \sum_{\mathbf{p}_i\in \boldsymbol{\mathcal{P}}} \min_{s_k\in\mathcal{S}} \|\mathbf{p}_i-s_k\|^2\\ &+  \frac{1}{|\mathcal{S}|} \sum_{s_k\in\mathcal{S}} \min_{\mathbf{p}_i\in\boldsymbol{\mathcal{P}}} \|\mathbf{p}_i-s_k\|^2,\vspace*{-2.5mm} \label{eq:CD}
\end{align}
The resulting point set will thus lie close to (and spread out on) the target surface. 

What sets our PoNQ apart is the additional (local) geometric information attached to each point $\mathbf{p}_i$ --- and the properties of the PoNQ mesh extracted from these points and their associated geometric data.
% \nm{Question about notation: should the font of Q match the font of P for easier understanding? And possibly put P in bold? Right now P and S look the same which might be confusing} \md{No idea what you mean. It's all in mathbf, what do you want? a capital P? The sets are in mathcal.}
Indeed, we enrich each point $\mathbf{p}_i\!\in\!\boldsymbol{\mathcal{P}}$ with a normal $\mathbf{n}_i$ and a QEM matrix $\textbf{Q}_i$. Denoting $V(\mathbf{p}_i)$ the Voronoi cell of $\mathbf{p}_i$ (i.e., the locations in $\mathbb{R}^3$ for which $\mathbf{p}_i$ is the closest from the set of all points $\{\mathbf{p}_k\}_{k=1}^m\!\coloneqq\mathcal{P}$, see~\cite{aurenhammer_voronoi_1991}), $\mathbf{n}_i$ represents the average of the sample normals $n(s_k)$ for all the samples $s_k$ contained within $V(\mathbf{p}_i)$ (see Figure~\ref{fig:summary_method}), i.e., \vspace*{-2mm}
\begin{equation}
    \mathbf{n}_i = \frac{1}{|\mathcal{S}\!\cap\! V\!(\mathbf{p}_i)|} \sum_{s_k \in \,\mathcal{S}\cap V\!(\mathbf{p}_i)} n(s_k).\vspace*{-2mm}
\end{equation}
Similarly, $\mathbf{Q}_i$ is assembled using Eqs.~\eqref{eq:sumsAbc} and~\eqref{eq:qem} using the tangent planes implied by each sample (and its normal) within $V(\mathbf{p}_i)$, i.e., $\textbf{Q}_i$ is the the QEM matrix such that 
\vspace*{-2mm}
\begin{equation}
    [x, 1]^t \,\mathbf{Q}_i\, [x, 1] = \sum_{s_k \in \mathcal{S}\cap V(\mathbf{p}_i)} d^2_{s_k, n(s_k)}(x). 
\vspace*{-3mm}
\end{equation}
Note that these additional geometric variables thus describe  the local geometry of the intersection of the input surface with the Voronoi cell of their associated point; points with no input samples within their Voronoi cell are simply discarded.
As explained in Section~\ref{sec:related}, each matrix $\mathbf{Q}_i$ implies, through its sub-matrices $\mathbf{A}_i$ and $\mathbf{b}_i$, an optimal location $\mathbf{v^*}\!\coloneqq\!\mathbf{A}_i^{-1}\mathbf{b}_i$ with respect to the input surface, hinting at the fact that storing $\mathbf{v^*}$ instead of  $\mathbf{b}_i$ is a possible alternative, which we will use in the learning context in the next section.
Finally, we will extract our final PoNQ mesh by first computing the Delaunay tetrahedralization of all the optimal points $\mathbf{v^*}$, followed by a round of tagging of tetrahedra derived from the Crust algorithm and complemented by a graph cut. before the extraction of a subset of the Delaunay triangles forming the ouput. This phase, along with its guarantees, will be described in Sec.~\ref{sec:method_meshing}.

\begin{figure}[h!]
    \begin{subfigure}{.21\textwidth}
      \centering
      \includegraphics[width=\linewidth]{figs/summary/summary_method.pdf} 
        \caption{\textit{Optimized PoNQ point set}}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.21\textwidth}
      \centering    
      \includegraphics[width=\linewidth]{figs/summary/summary_method2.pdf}
    \caption{\textit{PoNQ meshing}}
    \end{subfigure}%\vspace*{-2mm}
\caption{2D illustration of PoNQ. (a) A ground truth shape (blue line) is represented with points $\mathbf{p}_i$, normals $\mathbf{n}_i$ and quadrics $\mathbf{Q}_i$. (b) The PoNQ mesh (black solid lines) is the union of labeled tetrahedra from the Delaunay triangulation of the QEM-optimal vertices. It provides a better fit than simply interpolating the points (black dotted lines). \vspace*{-6mm}}
  \label{fig:summary_method}
\end{figure}

\subsubsection{Learning with PoNQ} 
\label{sec:method_learning}

We demonstrate the benefits of PoNQ in a learning-based context by applying it to the problem of mesh reconstruction from Signed Distance Fields (SDF) (see Figure~\ref{fig:cnn_summary}). As shown in several recent works~\cite{chen_neural_2021, chen_neural_2022, maruani_voromesh_2023}, this task is especially interesting as it enables the training of a \textit{local} model that can generalize to shapes across different categories from the training set. 
\begin{figure}[hbt]
  \centering
  \includegraphics[width=\linewidth]{figs/summary/summary.pdf}\vspace*{-2mm} 
\caption{Overview of our learning pipeline.\vspace*{-4mm}} 
  \label{fig:cnn_summary}
\end{figure}

We use an architecture similar to NDC \cite{chen_neural_2022}, consisting of several convolutional neural networks (CNN). Unlike NMC (which uses eight points per voxel) and NDC (which uses only one), we can use an arbitrary number $P$ of predicted points per cell since our representation does not depend on a regular grid --- in practice, we found that $P\!=\!4$ can represent sub-voxel details nicely without requiring too large networks.
We use a shared 5-layer encoder that converts the $(N\!+\!1)^3$ input SDF grid 
%$I \!\in\! \mathbb{R}^{ (N+1)^3}$ ---used? 
into a $N^3$-sized grid of 128 features $F \!\in\! \mathbb{R}^{N^3 \times 128}$. These features are processed by five separate 6-layer decoders (which do not share weights) to predict the PoNQ point set  $\boldsymbol{\mathcal{P}}$, i.e.,  $P\!\times\!N^3$ points $ \mathbf{p}_i$, along with their normals $\mathbf{n}_i$ and QEM matrices $\mathbf{Q}_i$, to which we add a set $\mathcal{O}$ of $N^3$ binary ``occupancies'' $\mathbf{o}_i$ to mark the voxels containing the surface at inference time.

To stabilize the learning process and avoid having to perform inversions of learned matrices $\mathbf{Q}_i$, we do not store QEM matrices directly but only use the quadratic form $\mathbf{A}_i$ and the QEM-optimized vertex location $\mathbf{v^*}$ instead, from which one can reconstruct $\mathbf{Q}_i \!= \!\!\bigl(\! \begin{smallmatrix}\scriptstyle 
\mathbf{A}_i & -\mathbf{A}_i \mathbf{v}_i^*\\
- (\mathbf{A}_i \mathbf{v}_i^*)^t & 0 \!\!
\end{smallmatrix}\bigr)\!.$
Furthermore, we store instead of $\mathbf{A}_i$ a $3 \!\times\! 3$ upper triangular matrix $\mathbf{U}_i$ such that $\mathbf{A}_i \!=\! \mathbf{U}_i\mathbf{U}_i^t$ is the reversed Cholesky decomposition of $\mathbf{A}_i$ -- guaranteeing that $\mathbf{A}_i$ remains invertible.

We supervise our training with a collection of watertight shapes, each converted into a dense sampling $\mathcal{S}$. We preprocess the data by computing the ground-truth occupancy set $\mathcal{O}_{gt}$ of voxels containing samples, to which we restrict our loss terms (except for $L_\text{occ}$, which checks how well the trained occupancy set matches the ground-truth one),
At training time, we apply the sum of the following losses and backpropagate their gradients w.r.t. underlined variables: \vspace*{-2mm} 
%\nm{I would use $\| x \|$ for all vector/matrix realted losses but I'm not sure what's clearer}
%\md{i think it's not bad to remind people of vector vs matrix; but it's a minor point anyway.}
\newcommand{\requiresgrad}[1]{\underline{#1}}
\allowdisplaybreaks
\begin{align}
&L_{\operatorname{CD}}(\theta) = \operatorname{CD}(\requiresgrad{\boldsymbol{\mathcal{P}}}(\theta), \mathcal{S}) \quad (\text{\emph{see Eq.~\eqref{eq:CD}}})\\
 &L_\mathbf{n}(\theta) = \tfrac{1}{|\boldsymbol{\mathcal{P}}(\theta)|} \sum_{\mathbf{p}_i \in \boldsymbol{\mathcal{P}}(\theta)}  \sum_{s_k\in \mathcal{S}\cap V(\mathbf{p}_i)} |\requiresgrad{\mathbf{n}_i} - n(s_k)|^2 \\
 &L_\mathbf{A}(\theta) \!= \!\tfrac{1}{|\boldsymbol{\mathcal{P}}(\theta)|} \!\!\textstyle\sum\limits_{ \substack{\mathbf{p}_i\\[-1.25mm] \rotatebox{270}{$\scriptscriptstyle \in$}\\ \scriptscriptstyle\boldsymbol{\mathcal{P}}(\theta)}}   \textstyle\sum\limits_{\substack{s_k\\[-1.25mm] \rotatebox{270}{$\scriptscriptstyle \in$}\\ \scriptscriptstyle\mathcal{S}\cap V(\mathbf{p}_i)}} \!\! \!\| \requiresgrad{\mathbf{U}}_i \requiresgrad{\mathbf{U}}_i^t -  n(s_k) n(s_k)^t  \|_{\scriptscriptstyle \text{Frob}}^2 \\
 &L_{\mathbf{v^*}}(\theta) = \tfrac{1}{|\boldsymbol{\mathcal{P}}(\theta)|} \sum_{\mathbf{v}_i^\textbf{*}(\theta)} 
 \sum_{\substack{s_k\\[-1.25mm] \rotatebox{270}{$\scriptscriptstyle \in$}\\ \scriptscriptstyle\mathcal{S}\cap V(\mathbf{p}_i)}}
 | n(s_k)^t (\requiresgrad{\mathbf{v}_i^\textbf{*}} - s_k)|^2 \\
&L_\text{reg}(\theta) = \tfrac{1}{|\boldsymbol{\mathcal{P}}(\theta)|} \sum_{\mathbf{p}_i \in \boldsymbol{\mathcal{P}}} | \requiresgrad{\mathbf{v}_i^\textbf{*}}-\mathbf{p}_i|^2 \\
 % &L_{occ}(\theta) = \operatorname{BCE}(\requiresgrad{\boldsymbol{\mathcal{O}}}(\theta),\mathcal{O}_\text{gt}) \vspace*{-1mm}
 &L_\text{occ}(\theta) =\| \requiresgrad{\boldsymbol{\mathcal{O}}}(\theta) - \mathcal{O}_\text{gt}\|^2. \vspace*{-5mm}
\end{align}

In the order in which they are listed above, these losses were designed to: help spread out the point set $\mathcal{P}$ and best fit the inputs; enforce that each normal is the mean normal of the local sample normals; enforce that the quadratic forms $\mathbf{A}_i$ corresponds to the proper submatrix of the QEM of the local samples and normals around point $\mathbf{p}_i$; enforce, similarly, that $\mathbf{v}_i^\textbf{*}$ minimizes the sum of squared distance to the local tangent planes around point $\mathbf{p}_i$; regularize (with a very small coefficient) the positions of the optimal points $\mathbf{v}_i^\textbf{*}$ in flat regions --- as in this case, any point on this flat region is optimal in theory, so we force it to stay close to $\mathbf{p}_i$; and make sure that we match the ground-truth occupancy set.\vspace*{-1mm} 

\subsubsection{Meshing our representation}
\label{sec:method_meshing}

The choices we made to design our QEM-based representation allow for a simple meshing approach, inspired by computational geometry to ensure robustness: due to the local optimality of the position $\mathbf{v}_i^\textbf{*}$ (in particular, their ability to capture corners and sharp features), our output mesh will be produced by filtering the triangle facets of a 3D Delaunay triangulation of the optimal positions $\mathbf{v}_i^\textbf{*}$.

Given the PoNQ data produced by a trained network, we first describe how a PoNQ mesh is extracted, before providing an extension to handle meshes with boundaries as well. 

\tightpara{0. Pre-processing} We first  normalize the quadrics by dividing them by their largest eigenvalue. While this technically changes their meaning (they now measure Euclidean distances \emph{up to a multiplicative constant}), it also removes the possible bias due to variable sampling density. Additionally, a bounding box $B$ of all the points $\mathbf{v}_i^\textbf{*}$ is computed.

\tightpara{1. \!Triangulation of QEM optimal positions.\!\!}
We then compute the Delaunay tetrahedralization of all $\mathbf{v}_i^\textbf{*}$, to which we add eight ``protective'' points defined as the corners of the bounding box $B$: all the adjacent tetrahedra to these protective points will be guaranteed to be outside of the shape we wish to reconstruct.  
The next two steps will tag each of the other tetrahedra as either \emph{inside} or \emph{outside} based on local geometric information, so that \emph{our final PoNQ mesh will be simply the triangle mesh forming the boundary between the inside and outside regions}, ensuring watertightness and no self-intersections by design. 

\tightpara{2.\! Tagging obvious inside/outside tetrahedra.}
We first tag all the tetrahedra adjacent to the eight protective point as \emph{outside}. Tagging the other tetrahedra seems difficult, but by leveraging the ideas put forth in the Crust algorithm~\cite{amenta_new_1998}, we note that the location of the circumcenter of a Delaunay thetrahedron whose four vertices are on the surface to mesh (which is the case we are in) can often determine the insideness or outsideness of this tetrahedron --- corresponding to whether this circumcenter is on the inside (resp. outside) medial axis. We use a similar approach here, except that our Delaunay vertices have additional information to help us: we also know a local normal $\mathbf{n}_i$ in the vicinity of each vertex $\mathbf{v}_i^\textbf{*}$. Thus each vertex along with its assigned normal defines an oriented plane, forming the boundary between the outside half-space (the one pointed by the normal) and the inside half-plane. Using this local test to determine inside/outside, we tag a tetrahedron as \emph{outside} (resp., \emph{inside}) if both its circumencenter and barycenter are determined to be in the outside (resp., inside) half-space of each of the four vertices. 
Then, we go through every (non-protective) vertex which already has at least one tagged adjacent tetrahedron. If such a vertex do not have any adjacent \emph{outside} (resp., \emph{inside}) tetrahedron, we pick its untagged adjacent tetrahedron with the smallest edge; if the size of this smallest edge is below a certain threshold (i.e., we are not in a very sparse region of the domain), we then tag this selected tetrahedron as \emph{outside} (resp., \emph{inside}). 
The rationale behind this last round of tagging is that we know that all vertices of our 3D Delaunay triangulation are \emph{on} the surface, so unless the smallest teterahedron is too big (in this case, there is clearly a large uncertainty), we can safely tag it to be on the opposite side of the surface than the side that the other tags had already determined. While this tagging procedure can, at times, tag \emph{all} tetrahedra, there are often a few remaining tetrahedra, typically caused by the presence of near sharp features or thin structures, that are too ambiguous to tag. We now need to lift the remaining uncertainty based on PoNQ. 
\tightpara{3.\! Finishing up triangle selection.\!}
Delaunay-based meshing approach (like \emph{Crust}) require a dense point sampling (formally, an $\epsilon-$sampling) to offer topological and geometric guarantees, which is not compatible with our desire to deal with thin structures, sharp features and corners --- and this is the main reason why our earlier phase often ends up not providing a clear tag for \emph{every} tetrahedra. To finish our tetrahedron tagging based on the ones we already have, we propose to use a graph cut approach, inspired by existing spectral graph partitioning~\cite{kolluri_spectral_2004}. 
For each Delaunay triangle $T$ between two adjacent tetrahedra for which \emph{at least} one of them is still undetermined, we compute a likelihood score $S(T)$ that evaluates how confident we are that this triangle is to appear on the final output mesh. We propose a score which evaluates the  fitness of $T$ based on the local PoNQ normals and the local PoNQ quadrics matrices: \vspace*{-2.5mm}
\[S(T) = S_\mathbf{n}(T) + h S_\mathbf{Q}(T)\vspace*{-2.5mm}\] (with $h$ set as the squared inverse of the edge length of the SDF grid), where: \vspace*{-2.5mm}
\begin{align}
S_n(T) &=  \bigl(\tfrac2\pi \textstyle\sum\limits_{\mathbf{v}_i^\textbf{*} \in T} \arccos(n_{T}^t \,\mathbf{n}_i) \bigr)^2   \\[-1mm]
S_Q(T) &=  \textstyle\sum\limits_{ \mathbf{v}_i^\textbf{*} \in T}  \textstyle\sum\limits_{\substack{ \mathbf{v}_j^\textbf{*} \in T \\ i \neq j}} [\mathbf{v}_i^\textbf{*}, 1]^t \mathbf{Q}_i [\mathbf{v}_i^\textbf{*}, 1]\\[-9mm]
\label{eq:meshing}
\end{align}
We can now tag the remaining undetermined tetrahedra with a definite  \emph{inside} or \emph{outside} label: we compute a minimum cut of the Voronoi graph (in which each dual of a tetrahedron is a node, and each dual of a Delaunay triangle face is an edge) using the already-tagged "inside" ones as a source and the "outside" one as a drain, and each edge weight between two tetrahedra (with a common face $T$)  set to the score $S(T)$.
Since most of tetrahedra are already tagged, we can merge Voronoi edges between marked tetrahedra to accelerate computations. We now just have to extract the final \textit{PoNQ mesh} as the triangle mesh forming the boundary between the inside and outside regions. 

\tightpara{Extension: Open surfaces}
\label{sec:boundary}
With minor modifications, PoNQ can output surfaces with boundaries as well. Within an optimization context, we simply compute a ``boundary sampling'' $\mathcal{S}_b$ of the input surface boundaries, and duplicate it to create a sampling $\mathcal{S}'_b$ where we just rotate all the normals by $\pi/2$ around the boundary. Changing $\mathcal{S}$ into $\mathcal{S}\cup\mathcal{S}_b\cup\mathcal{S}_b'$ will thus enforce that all the QEM matrices on the boundaries will generate elongated ellipsoids aligned with the local boundary. Meshing can proceed as before, but the output mesh will automatically close the holes; so we further cull any triangle $T$ of the extracted mesh for which the anisotropy of the QEM of each of its vertices is above a threshold. In practice, we measure the anisotropy through the ratio $r_i \!=\! \frac{\lambda_2}{\lambda_1}$ of the two largest eigenvalues of the matrix $\mathbf{A}_i$. See Fig.~\ref{fig:summary} and the supplemental material for results.

%\begin{align}
%S_{\textit{open}}(T) = \Pi_{ a \in T }  \vmathbb{1}_{\frac{\lambda_{a, 2}}{\lambda_{a, 1}} > \alpha_b}  
%\end{align}

